Optimal design of Piezoelectric Energy Harvesters for bridge infrastructure: Effects of Location and Traffic Intensity on Energy Production

Piezoelectric energy harvesters (PEHs) can be used as an additional power supply for a Structural Health Monitoring (SHM) system. Its design can be optimised for the best performance; however, the optimal design depends on the input vibration, e.g. acceleration of a bridge due to wind loads and passing traffic. In previous studies, we have shown that optimal design tunes to some predominant frequency of the signal spectrum. However, our previous study was limited to a single location of a PEH on a bridge. In this work, we extend the rigorous optimisation framework to include the effect of the PEH's location. The optimisation framework uses the PEH plate model discretised by IsoGeometric Analysis (IGA) and coupled with the Particle Swarm Optimisation algorithm to find the designs with maximum energy outputs for many acceleration histories, extracted from the recorded dynamic response data of a real cable-stayed bridge in Australia. Then, clustering is performed to find several best candidates for the entire bridge. An additional study is performed to quantify the effect of traffic intensity on the produced energy. It is shown that variation in traffic volume throughout the 24hr time window leads to variation in optimal PEH designs. The study concludes the impact of location and traffic on energy harvesting by identifying the optimal PEH design and placement throughout the bridge structure. The results indicate that the key factors of maximising energy harvesting efficiency are related to the input excitation and the mode of vibration being excited. The position of maximum displacement in the vibration mode corresponds to the best location for energy harvesting. Also, the change in traffic intensity affects the amount of convertible mechanical energy and also directs the fundamental frequency of a PEH to shift within a specific range of frequencies to achieve the highest energy conversion.

==> Sections/section5.tex <==
\label{4.3}
Clustering is to group multiple optimal designs at each location obtained in the previous section according to equipment characteristics and identify candidates, which is a key prerequisite for designing the best PEH at all locations of the entire bridge structure. Since the natural frequencies of the previously mentioned optimal devices tend to be tuned to one of the resonant frequencies of the bridge structure, the clustering will be performed according to the fundamental frequency characteristics of the geometric configuration. In this section, the $k-$means method \cite{ex38}, which has applicability and efficiency for classifying geometrically distinct clusters, is employed to group shape-optimized geometric designs. As an unsupervised learning algorithm, $k-$means identifies the class of the sample and the centroid of each cluster by iteratively adjusting the distance between each sample element (the best design) and the centroid to a minimum value. The clustering category value $k$ is the key to measure the sample similarity and clustering effect, so Silhouette Coefficient \cite{ex39} is employed to evaluate the dispersion of clusters. As a variable to measure the clustering effect of all samples, the clustering effect is proportional to the $S$ value reflecting the distance of the samples in the cluster, and the calculation formula is as follows.
\begin{equation}
    S=\frac{\left ( b-a\right )}{max\left ( a,b\right )}\in \left [ -1,1\right ]
    \label{e5.3}
\end{equation}
where $a$ is the average distance between the sample element and other samples in the same cluster, and $b$ is the average distance between the sample element and other clusters.

Then candidates at each location represented by centroids obtained after performing $k-$means on all optimal designs are identified to compare the energy collected from 24-hour continuous acceleration windows in order to filter the best geometry configuration options.

\subsection{Clustering and Candidate Identification}\label{4.3.1}
As mentioned in Section \ref{4.2.2}, the clustering in this work is performed according to the fundamental frequency of the device affected by the input excitation environment. By searching and detailed partitioning of all optimally designed natural frequencies, representative frequency characteristics are listed in Figure \ref{5.15}, and then the design space of PEH over the entire bridge structure is classified based on the detailed frequency partitioning and displayed in In the variable space consisting of the four parameters $L, R, H, l$ (Figure \ref{5.16}).
\begin{figure}[H]
	\centering
	\includegraphics[width=1\linewidth]{Figures/5.15.png}
	\caption{Detailed division based on the natural frequencies of optimal designs.}
	\label{5.15}
\end{figure}
\begin{figure}[H]
	\centering
	\includegraphics[width=1\linewidth]{Figures/5.16.png}
	\caption{Distribution of PEH design in parameter space ($L, R, H, l$).}
	\label{5.16}
\end{figure}

From the error comparison of 12 natural frequencies presented in Figure \ref{5.17}, it can be seen that the clustering effect between different categories is significant. In addition, it can be observed that the main standard deviation occurs in the space of the shape variable $l$, especially between the first two natural frequencies, which verifies that the dispersion of the variable $l$ mainly originates from the adjustment of the energy absorbed by the device from the first and second vibrational modes introduced by Peralta et al. \cite{ex35}. But $L$ is the main geometric shape parameter that affects the energy harvesting efficiency of PEHs, and it can be seen from Figure \ref{5.17} that the clustering performed based on the input signal and device shape is ideal.
\begin{figure}[H]
	\centering
	\includegraphics[width=1\linewidth]{Figures/5.17.png}
	\caption{Error bar graph for different natural frequencies.}
	\label{5.17}
\end{figure}

However, due to the excessively detailed division of frequencies, a large number of candidates are generated, which violates our design philosophy, so the division criteria are further changed to achieve reasonable candidate identification, as shown in Figure \ref{5.18}. Figure \ref{5.19} illustrates that geometric parameter clustering of optimal PEHs based on updated natural frequency classes is acceptable.
\begin{figure}[H]
	\centering
	\includegraphics[width=1\linewidth]{Figures/5.18.png}
	\caption{Updated detailed division of natural frequencies.}
	\label{5.18}
\end{figure}
\begin{figure}[H]
	\centering
	\includegraphics[width=1\linewidth]{Figures/5.19.png}
	\caption{Error bar graph for updated different natural frequencies.}
	\label{5.19}
\end{figure}

Therefore, the clustering work is extended to the optimal design space for each location to identify candidates under the same framework, so the following steps take S20 as an example. The 24 optimal devices at S2 obtained in Section \ref{4.2.2} are shown in Figure \ref{5.20}. It should be noted that for some locations with a high degree of aggregation of device configurations, such as S10, only one cluster is identified (Figure \ref{5.21}). 
\begin{figure}[H]
	\centering
	\includegraphics[width=1\linewidth]{Figures/5.20.png}
	\caption{Expression of the 24 optimal devices at S2 in the design space.}
	\label{5.20}
\end{figure}
\begin{figure}[H]
	\centering
	\includegraphics[width=1\linewidth]{Figures/5.21.png}
	\caption{Expression of the 24 optimal devices at S10 in the design space.}
	\label{5.21}
\end{figure}

While for locations with high device configuration dispersion, such as S2, the number of clusters is determined according to the silhouette coefficient, as shown in Figure \ref{5.22}, the largest silhouette value corresponds to the optimal number of clusters of 3. It is also worth mentioning that in the spatial representation of the design parameters, samples in different clusters are represented by different colors, and the centroids denoted by crosses are candidates for each cluster (Figure \ref{5.23}).
\begin{figure}[H]
	\centering
	\includegraphics[width=0.7\linewidth]{Figures/5.22.png}
	\caption{Silhouette Coefficient for the optimal geometries at S2.}
	\label{5.22}
\end{figure}
\begin{figure}[H]
	\centering
	\includegraphics[width=1\linewidth]{Figures/5.23.png}
	\caption{Expression of the optimal geometry among the three clusters in the design space.}
	\label{5.23}
\end{figure}

The spectral features of each candidate are presented in Figure \ref{5.24}. Finally, the 432 optimal PEH geometries over the entire bridge structure are sorted into 36 candidates, and their energy harvested in a 24-hour continuous window is evaluated in the next step.
\begin{figure}[H]
	\centering
	\includegraphics[width=1\linewidth]{Figures/5.24.png}
	\caption{FRF responses of four candidates.}
	\label{5.24}
\end{figure}

In addition, the number of clusters at each location shows that the optimal geometric design at edge locations is more discrete, which is consistent with the results in Section \ref{4.2.2}, since other vibration modes start to be excited when there is a window with enough vehicles passing the bridge. The optimization is performed by synchronizing the fundamental frequency of the device with the dominant frequencies of the acceleration spectrum, including the peaks with the highest or widest amplitude. For locations such as S10 where the bridge dynamic response is large under the first vibration mode, the most energy can be absorbed from the first mode, while for PEH designs at the edge panels, the generation of energy in other modes is adjusted by tuning to other natural frequencies to maximize harvesting efficiency. Thus, time series windows with different degrees of excitation induce discreteness of the optimal geometry at some locations, further explanations will be discussed in the last section.



\subsection{Distribution of Optimal Devices and Locations}\label{4.3.2}
To identify the best options for PEH geometric design at each location on the cable-stayed bridge, the energy harvesting capabilities of the candidates extracted in Section \ref{4.3.1} under a 24-hour continuous acceleration signal input are evaluated and presented in Figure \ref{5.25}, where the color represents the PEH configuration with the natural frequency in Figure \ref{5.24}, the size of the circle is proportional to the collected energy.
\begin{figure}[H]
	\centering
	\includegraphics[width=1\linewidth]{Figures/5.25.png}
	\caption{Energy harvesting capabilities of the candidates.}
	\label{5.25}
\end{figure}

Figure \ref{5.26} shows the best PEH geometric design at each position. Combining with the modal shape (Figure \ref{5.27}a), it can be seen that the best design at the position with large deformation in the first bending moment mode tends to have similar frequency characteristics to the first vibration mode. Therefore, a consistent phenomenon is exhibited for the optimized designs from S5 to S16. For the optimal design at the edge panels (S17, S18, S19 and S20), due to the small displacement in the first bending moment mode, which results in almost no energy harvesting from the first vibration mode, while Figure \ref{5.27}b illustrates that the PEH mounted at edges can absorb the energy from the second mode through geometric optimization, so the best candidates at the edge panel are the devices tuned to the second natural frequency.
\begin{figure}[H]
	\centering
	\includegraphics[width=1\linewidth]{Figures/5.26.png}
	\caption{Expression of the best PEH geometric design at each location in the parameter space.}
	\label{5.26}
\end{figure}
\begin{figure}[H]
	\centering
	\includegraphics[width=0.95\linewidth]{Figures/5.27.png}
	\caption{Illustration of the first two bending modes corresponding to the first two natural frequencies obtained from field test \cite{ex37}.}
	\label{5.27}
\end{figure}

In addition, the best candidates at S2 and S3 indicate that the fundamental frequency of the PEH device can not only improve energy harvesting efficiency by matching the amplitude peaks of the acceleration spectrum but also can be tuned to a certain frequency range to harvest energy from multiple vibration modes, which depends on the deformation mode of the structure and the strength of the external excitation. Although positions 2 and 3 have the highest displacements in the second mode, due to the characteristics of the traffic flow under the real operating conditions of the cable-stayed bridge in this work, the first mode is more inclined to be excited, and the first acceleration peak is higher than the second peak. Therefore, the energy harvested from the first mode is non-negligible, so the optimization of the PEH geometry maximizes the energy absorbed from the first two modes by synchronizing the natural frequencies between the first two frequencies.

Finally, from the best candidates at all positions summarized in Figure \ref{5.28}, it can be concluded that the proposed optimization framework can identify the geometric configuration and installation position of a limited number of PEHs on the bridge to achieve the optimization of energy harvesting performance.
\begin{figure}[H]
	\centering
	\includegraphics[width=1\linewidth]{Figures/5.28.png}
	\caption{Distribution positions of best candidates over the entire structure and energy representations collected under the 24-hour continuous window.}
	\label{5.28}
\end{figure}

==> Sections/section6.tex <==
\label{4.4}
As mentioned before, the strength of the external excitation is also a key factor affecting the energy harvesting efficiency and the optimal geometry of the device. For example, Section \ref{4.2.1} concludes that the optimal shape of PEH equipment tends to be centralized in the absence of vehicle driving, indicating the effect of events on the discreteness of PEHs design. Therefore, this section explores how traffic affects energy generation and shape optimization of devices by identifying the number of vehicles in consecutive windows.

Figure \ref{5.29} shows the number of vehicles identified from a typical acceleration time signal with a threshold of $0.2m/s^2$ of acceleration due to a passing vehicle. The energy harvested across the bridge in 24 one-hour consecutive windows from the same day is shown in Figure \ref{5.30}, illustrating that traffic volume is proportional to energy output. Therefore, this study is extended to the energy output induced by single-event excitation, and the results show that each vehicle passing through the bridge can provide about 339 $\mu J$ of energy at one installation node (such as S9), which corresponds to the energy output of each vehicle (60-565 $\mu J$) proposed by Zhang et. al \cite{ex40}. However, related research needs further refinement, such as exploring the influence of vehicle model, wheelbase, driving direction, speed and distance on energy harvesting.
\begin{figure}[H]
	\centering
	\includegraphics[width=0.95\linewidth]{Figures/5.29.png}
	\caption{Number of vehicles identified in four one-hour consecutive windows.}
	\label{5.29}
\end{figure}
\begin{figure}[H]
	\centering
	\includegraphics[width=0.95\linewidth]{Figures/5.30.png}
	\caption{Energy harvested from 24 one-hour time series windows. (The grey bars are the energy collected by the four example windows.)}
	\label{5.30}
\end{figure}

In addition, the strength of the traffic excitation can interfere with the geometric design of the optimal equipment. Figure \ref{5.32} shows the spectral characteristics of the optimal device excited at S2 in three time-series windows with different traffic volumes (Figure \ref{5.31}). It can be seen that the three excitation states with different numbers of vehicles correspond to three different fundamental frequencies of the equipment: when there are very few passing vehicles, only the first mode is excited, and the device fundamental frequency is optimized to the first frequency; when the number of vehicles starts to increase, other modes start to be excited, and the optimal equipment is adjusted to increase the energy generated from the second mode; when the traffic volume is high, the second mode is fully excited, and the maximum energy harvesting capability is achieved by tuning the device to the second frequency.
\begin{figure}[H]
	\centering
	\includegraphics[width=0.95\linewidth]{Figures/5.31.png}
	\caption{Three representative time series windows.}
	\label{5.31}
\end{figure}
\begin{figure}[H]
	\centering
	\includegraphics[width=1\linewidth]{Figures/5.32.png}
	\caption{Spectral characteristics of the optimal device excited at S2 for three time series windows.}
	\label{5.32}
\end{figure}

It is worth noting that the second deformation mode mentioned in Section \ref{4.3.2} shows that S2 can absorb the most energy from the second vibration mode. The reason why the best option for S2 is not a device that matches the second frequency is that the operating environment of the cable-stayed bridge used in this work generally does not have high flow, so events that can sufficiently excite the second mode are not enough to dominate the optimization of geometric configuration.

Therefore, the structural dynamic response of infrastructure and the characteristics of traffic intensity in operating conditions are the key influencing factors for performing PEH shape optimization and identifying the optimal location.
